End-to-End Speech Recognition With Joint Dereverberation Of Sub-Band Autoregressive Envelopes

The end-to-end (E2E) automatic speech recognition (ASR) systems are often required to operate in reverberant conditions, where the long-term sub-band envelopes of the speech are temporally smeared. In this paper, we develop a feature enhancement approach using a neural model operating on sub-band temporal envelopes. The temporal envelopes are modeled using the framework of frequency domain linear prediction (FDLP). The neural enhancement model proposed in this paper performs an envelope gain based enhancement of temporal envelopes. The model architecture consists of a combination of convolutional and long short term memory (LSTM) neural network layers. Further, the envelope dereverberation, feature extraction and acoustic modeling using transformer based E2E ASR can all be jointly optimized for the speech recognition task. The joint optimization ensures that the dereverberation model targets the ASR cost function. We perform E2E speech recognition experiments on the REVERB challenge dataset as well as on the VOiCES dataset. In these experiments, the proposed joint modeling approach yields significant improvements compared to the baseline E2E ASR system (average relative improvements of 21% on the REVERB challenge dataset and about 10% on the VOiCES dataset).

==> Tables/Table_3_e2e_vs_h.tex <==
\begin{table}[t!]
\caption{Word Error Rate (\%) in REVERB dataset for different dereverberation neural model architectures with BF-FDLP features.}
\resizebox{\columnwidth}{!}{
%\centering
\begin{tabular}{@{}l|ccc|ccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\ architecture\end{tabular}}}} & \multicolumn{3}{c|}{\textbf{Dev}}                                              & \multicolumn{3}{c}{\textbf{Eval}} &                                             \\ \cmidrule(l){2-7} 
\multicolumn{1}{c|}{}                                                                                   & \multicolumn{1}{l}{\textbf{Real}} & \multicolumn{1}{l}{\textbf{Simu}} & \multicolumn{1}{l|}{\textbf{Avg}} & \multicolumn{1}{l}{\textbf{Real}} & \multicolumn{1}{l}{\textbf{Simu}} & \multicolumn{1}{l}{\textbf{Avg}} \\ \midrule
4-CNN + 4-TRANS                                                                                          & 14.8                     & 9.8                      & 12.3                     & 11.3                     & 9.7                      & 10.5                    \\
2-CNN + 4-TRANS                                                                                           & 15.1                     & 10.7                      & 12.9                     & 12.2                     & 9.9                      & 11.1                    \\
4-TRANS + POS                                                                                           & 14.3                    & 9.5                     & 11.9                      & 11.5                     & 9.3                      & 10.4                     \\ \hline
4-CNN + 2-LSTM                                                                                            & \textbf{11.4}                    & \textbf{7.7}                     & \textbf{9.5}                      & \textbf{9.5}                     & \textbf{7}                      & \textbf{8.2}                     \\ \bottomrule
% 4-CNN + 2-LSTM(Hybrid)                                                                                           & {14.4}                    & {5.3}                     & {9.9}                      & {12}                     & {6.8}                      & {9.4}                     \\
%\bottomrule
\end{tabular}}
\label{table:3_a}
\end{table}

==> Tables/Table_5_voices_with_agu.tex <==
\begin{table}[t!]
\centering
\caption{WER in VOiCES dataset for different features in End to End ASR using ESPnet, with Augmentation}
\begin{tabular}{l|c|c}
\toprule
\multirow{1}{*}{\textbf{Model Architecture}} & \multicolumn{1}{c|}{\textbf{Dev}}            & \multicolumn{1}{c}{\textbf{Eval}}            
                                      \\ \midrule
BF-FBANK                             &42.1              & 51.5         \\
BF-FDLP                            &39.9            & 49.4        \\
BF-FDLP + CLSTM derevb.                             &41.1           & 51        \\ \hline
~~~~~~~~~~~~~ + joint. (prop)                           & \textbf{}           & \textbf{}        \\
\bottomrule
\end{tabular}

\label{table:4}
\end{table}

==> Tables/table_with_param_rev.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Word Error Rate (\%) in REVERB dataset for dif-ferent  dereverberation  neural  model  architectures  with  BF-FDLP features.}
\label{table:3}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\ Architecture\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\ Parameters\\ (in Million)\end{tabular}}} & \multicolumn{3}{c|}{\textbf{DEV}} & \multicolumn{3}{c}{\textbf{EVAL}} \\ \cline{3-8} 
 &  & \multirow{2}{*}{\textbf{Real}} & \multirow{2}{*}{\textbf{Simu}} & \multirow{2}{*}{\textbf{Avg}} & \multirow{2}{*}{\textbf{Real}} & \multirow{2}{*}{\textbf{Simu}} & \multirow{2}{*}{\textbf{Avg}} \\
 &  &  &  &  &  &  &  \\ \hline
\begin{tabular}[c]{@{}c@{}}2 CNN + \\ Transformer\end{tabular} & 137.42 & 15.1 & 10.7 & 12.9 & 12.2 & 9.9 & 11.1 \\ \hline
\begin{tabular}[c]{@{}c@{}}4 CNN + \\ Transformer\end{tabular} & 54.7 & 14.8 & 9.8 & 12.3 & 11.3 & 9.7 & 10.5 \\ \hline
\begin{tabular}[c]{@{}c@{}}Linear Layer + \\ Transformer\end{tabular} & 19.8 & 14.3 & 9.5 & 11.9 & 11.5 & 9.3 & 10.4 \\ \hline
\begin{tabular}[c]{@{}c@{}}4 CNN + \\ 2 LSTM\end{tabular} & \textbf{14.5} & \textbf{11.4} & \textbf{7.7} & \textbf{9.5} & \textbf{9.5} & \textbf{7} & \textbf{8.2} \\ \hline
\end{tabular}%
}
\end{table}

==> fig.tex <==
\begin{figure*}[t!]
  \centering
  \includegraphics[width=\textwidth]{asru_2021_spectrogram_plot.pdf}
      \caption{Comparison of spectrograms, FDLP spectrogram for clean (near-room), reverberant speech (far-room) and reverberant speech (far-room) after the proposed dereverberation approach. The recordings are from the REVERB Challenge test dataset.}
      \vspace{-0.2cm}
  \label{fig:SSAR_Spectrogram}
\end{figure*}
% \begin{figure*}[t!]
%   \centering
%   \includegraphics[width=\textwidth,height=4cm]{icassp_plot_env.pdf}
%       \caption{Comparison of temporal envelopes, FDLP envelopes for clean, reverberant speech and reverberant speech after proposed joint learning based dereverberation, recordings from the REVERB Challenge dataset.}
%       \vspace{-0.5cm}
%   \label{fig:env_enhancement}
% \end{figure*}
